"You are grounded!": Latent Name Artifacts in Pre-trained Language Models

Pre-trained language models (LMs) may perpetuate biases originating in their training corpus to downstream models. We focus on artifacts associated with the representation of given names (e.g., Donald), which, depending on the corpus, may be associated with specific entities, as indicated by next token prediction (e.g., Trump). While helpful in some contexts, grounding happens also in under-specified or inappropriate contexts. For example, endings generated for `Donald is a' substantially differ from those of other names, and often have more-than-average negative sentiment. We demonstrate the potential effect on downstream tasks with reading comprehension probes where name perturbation changes the model answers. As a silver lining, our experiments suggest that additional pre-training on different corpora may mitigate this bias.

==> 08-conclusion.tex <==
Firth said ``you shall know a word by the company it keeps'' \cite{firth1957synopsis}, but the company of given names often relates to specific named entities with this name. We showed this is prevalent in pre-trained LMs, especially ones trained on web text, and demonstrated the effect on downstream tasks. Although we focused primarily on high-frequency names, it is interesting to study such artifacts for non Euro-American names, which may not have dedicated tokens in the LM vocabulary and are likely to encode different types of biases. %\footnote{See the supplementary material for additional ethical considerations.}

%\footnote{See the supplementary material for additional ethical considerations.}
 
